A Non-Cooperative Multiple Access Game for Timely Updates

We consider a network of selfish nodes that would like to minimize the age of their updates at the other nodes. The nodes send their updates over a shared spectrum using a CSMA/CA based access mechanism. We model the resulting competition as a non-cooperative one-shot multiple access game and investigate equilibrium strategies for two distinct medium access settings (a) collisions are shorter than successful transmissions and (b) collisions are longer. We investigate competition in a CSMA/CA slot, where a node may choose to transmit or stay idle. We find that medium access settings exert strong incentive effects on the nodes. We show that when collisions are shorter, transmit is a weakly dominant strategy. This leads to all nodes transmitting in the CSMA/CA slot, therefore guaranteeing a collision. In contrast, when collisions are longer, no weakly dominant strategy exists and under certain conditions on the ages at the beginning of the slot, we derive the mixed strategy Nash equilibrium.

==> MSNE_3Player.tex <==
Figure~\ref{fig:payoff_3player} shows the payoff matrix corresponding to the strategic game $G$. Three $\AO$ nodes contend for the medium and can choose between pure strategies, transmit ($\mathcal{T}$) and idle ($\mathcal{I}$).

\begin{figure}[t]
\subfloat{\includegraphics[width = 0.48\textwidth]{Figures/Payoff_3players_v1.pdf}}
\enspace
\subfloat{\includegraphics[width = 0.49\textwidth]{Figures/Payoff_3players_v2.pdf}}
\caption{Payoff matrix with slot lengths and AoI values at the end of stage $1$ for the game $G$, when three $\AO$ nodes contend for the medium and can choose between transmit ($\mathcal{T}$) and idle ($\mathcal{I}$). Negative payoffs indicates that each node desires to minimize its utility.}
\label{fig:payoff_3player}
\end{figure}
\begin{lem}
The parameter vector $\vect{\tau} = [\tau_{1}^{*},\tau_{2}^{*},\tau_{3}^{*}]$ required to compute the mixed strategy Nash equilibrium $\phi^{*} = (\phi_{1}^{*},\phi_{2}^{*},\phi_{3}^{*})$, for the 3-player one-shot game $G$ shown in Figure~\ref{fig:payoff_3player} is
\begin{align*}
\tau_{1}^{*} &= \frac{\lsucc-\lidle-(\Delta_{02}+\Delta_{03}-\Delta_{01})}{3\lsucc-2\lcol-\lidle-(\Delta_{02}+\Delta_{03}-\Delta_{01})},\\
\tau_{2}^{*} &= \frac{\lsucc-\lidle-(\Delta_{01}+\Delta_{03}-\Delta_{02})}{3\lsucc-2\lcol-\lidle-(\Delta_{01}+\Delta_{03}-\Delta_{02})},\\
\tau_{3}^{*} &= \frac{\lsucc-\lidle-(\Delta_{01}+\Delta_{02}-\Delta_{03})}{3\lsucc-2\lcol-\lidle-(\Delta_{01}+\Delta_{02}-\Delta_{03})}.
\end{align*}
\textbf{Proof}: Suppose $\AO$ $1$, $\AO$ $2$ and $\AO$ $3$ transmits with probability $\tau_{1}$, $\tau_{2}$ and $\tau_{3}$, respectively. For $\AO$ $1$ to randomize, $EU_{1}(\T) = EU_{1}(\I)$, where
\begin{align*}
EU_{1}(\T) &= -(\tau_{2}\tau_{3} + \tau_{2}(1-\tau_{3}) + \tau_{3}(1-\tau_{2}))(\Delta_{01}+\lcol) - (1-\tau_{2})(1-\tau_{3})\lsucc,\\
EU_{1}(\I) &= -\tau_{2}\tau_{3}(\Delta_{01}+\lcol) + (\tau_{2}(1-\tau_{3}) + \tau_{3}(1-\tau_{2}))(\Delta_{01}+\lsucc) - (1-\tau_{2})(1-\tau_{3})(\Delta_{01}+\lidle).
\end{align*}
since $EU_{1}(\T) = EU_{1}(\I)$, we have
\begin{align}
\frac{\tau_{2}}{1-\tau_{2}} + \frac{\tau_{3}}{1-\tau_{3}} = \frac{\lsucc-\lidle-\Delta_{01}}{\lsucc-\lcol}.
\label{Eq:cond_1}
\end{align}
For $\AO$ $2$ to randomize, $EU_{2}(\T) = EU_{2}(\I)$, where
\begin{align*}
EU_{2}(\T) &= -(\tau_{1}\tau_{3} + \tau_{1}(1-\tau_{3}) + \tau_{3}(1-\tau_{1}))(\Delta_{02}+\lcol) - (1-\tau_{1})(1-\tau_{3})\lsucc,\\
EU_{2}(\I) &= -\tau_{1}\tau_{3}(\Delta_{02}+\lcol) + (\tau_{1}(1-\tau_{3}) + \tau_{3}(1-\tau_{1}))(\Delta_{02}+\lsucc) - (1-\tau_{1})(1-\tau_{3})(\Delta_{02}+\lidle).
\end{align*}
since $EU_{2}(\T) = EU_{2}(\I)$, we have
\begin{align}
\frac{\tau_{1}}{1-\tau_{1}} + \frac{\tau_{3}}{1-\tau_{3}} = \frac{\lsucc-\lidle-\Delta_{02}}{\lsucc-\lcol}.
\label{Eq:cond_2}
\end{align}
Similarly, for $\AO$ $3$ to randomize, $EU_{3}(\T) = EU_{3}(\I)$, where
\begin{align*}
EU_{3}(\T) &= -(\tau_{1}\tau_{2} + \tau_{1}(1-\tau_{2}) + \tau_{2}(1-\tau_{1}))(\Delta_{03}+\lcol) - (1-\tau_{1})(1-\tau_{2})\lsucc,\\
EU_{3}(\I) &= -\tau_{1}\tau_{2}(\Delta_{03}+\lcol) + (\tau_{1}(1-\tau_{2}) + \tau_{2}(1-\tau_{1}))(\Delta_{03}+\lsucc) - (1-\tau_{1})(1-\tau_{2})(\Delta_{03}+\lidle).
\end{align*}
since $EU_{3}(\T) = EU_{3}(\I)$, we have
\begin{align}
\frac{\tau_{1}}{1-\tau_{1}} + \frac{\tau_{2}}{1-\tau_{2}} = \frac{\lsucc-\lidle-\Delta_{03}}{\lsucc-\lcol}.
\label{Eq:cond_3}
\end{align}
\end{lem}
On solving~(\ref{Eq:cond_1})-(\ref{Eq:cond_3}), we get,
\begin{align*}
\tau_{1}^{*} &= \frac{\lsucc-\lidle-(\Delta_{02}+\Delta_{03}-\Delta_{01})}{3\lsucc-2\lcol-\lidle-(\Delta_{02}+\Delta_{03}-\Delta_{01})},\\
\tau_{2}^{*} &= \frac{\lsucc-\lidle-(\Delta_{01}+\Delta_{03}-\Delta_{02})}{3\lsucc-2\lcol-\lidle-(\Delta_{01}+\Delta_{03}-\Delta_{02})},\\
\tau_{3}^{*} &= \frac{\lsucc-\lidle-(\Delta_{01}+\Delta_{02}-\Delta_{03})}{3\lsucc-2\lcol-\lidle-(\Delta_{01}+\Delta_{02}-\Delta_{03})}.
\end{align*}

